Causal Dioramas: Controllable Video Generation, Revision and Editing via Intervention

Two centuries ago, an early cinema-like theater called the Diorama could already control its scenes at will. Today's video generation models produce videos of near-cinematic quality, yet they still lack this controllability. This limitation stems from the inherent semantic gap between text and pixels, since a prompt can describe a video only coarsely and leaves its details and relations beyond control. We bring this ability to video generation with Causal Dioramas, modules that decompose a video into a concept graph of variables that can be intervened on individually. Each instruction is translated into an intervention on the concept graph, modifying the specified concepts and their dependents. A connector then conveys this intervention to the video generator, which reuses the original noise to produce a counterfactual video while preserving all other content. Building on Causal Dioramas, we develop a unified framework for controllable generation, counterfactual revision of generated videos and editing of real videos. We outperform both open-source and commercial models in controllability on T2V-CompBench, CoVEBench and OpenVE-Bench.

==> tables/ablation.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{UAS}\tabAmax\tabAcw{IFS}\tabAmax\tabAcw{VRS}\tabAmax\tabAcw{VQR}\tabAmax\tabAcw{SEM}\tabAmax\tabAcw{00.000}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{MiniMax H3~\cite{minimax2026h3}}\tabAmax\tabAmw{w/o Causal Diorama}\tabAmax\tabAmw{MiniMax H3~\cite{minimax2026h3}}\tabAmax\tabAmw{w/o Causal Diorama}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{\textit{Revision}}\tabAmax\tabAmw{\textit{Editing}}\tabAmax\tabAmw{Method}
\tabAtabular{l|ccc|c|c}{%
\toprule
\tabAname{Method} & \tabAcell{UAS} & \tabAcell{IFS} & \tabAcell{VRS} & \tabAcell{VQR} & \tabAcell{SEM} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Revision}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{MiniMax H3~\cite{minimax2026h3}} & \tabAcell{40.9} & \tabAcell{60.2} & \tabAcell{65.3} & \tabAcell{4.23} & \tabAcell{97.1} \\
\tabAname{w/o Causal Diorama} & \tabAcell{77.4} & \tabAcell{90.0} & \tabAcell{88.5} & \tabAcell{4.36} & \tabAcell{75.0} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{79.5} & \tabAtile{tabAours}{\tabAcw}{c}{92.7} & \tabAtile{tabAours}{\tabAcw}{c}{89.7} & \tabAtile{tabAours}{\tabAcw}{c}{4.30} & \tabAtile{tabAours}{\tabAcw}{c}{95.3} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Editing}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{MiniMax H3~\cite{minimax2026h3}} & \tabAcell{62.0} & \tabAcell{78.7} & \tabAcell{81.0} & \tabAcell{4.11} & \tabAcell{91.4} \\
\tabAname{w/o Causal Diorama} & \tabAcell{78.0} & \tabAcell{91.2} & \tabAcell{88.6} & \tabAcell{4.26} & \tabAcell{55.5} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{79.8} & \tabAtile{tabAours}{\tabAcw}{c}{91.7} & \tabAtile{tabAours}{\tabAcw}{c}{90.1} & \tabAtile{tabAours}{\tabAcw}{c}{4.23} & \tabAtile{tabAours}{\tabAcw}{c}{93.5} \\
\bottomrule}
\caption{Ablation on CoVEBench. All variants use MiniMax H3 as the generator. Higher is better for all metrics.}
\label{tab:ablation}
\vspace{-12pt}
\end{table}


==> tables/ablation_causal.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{UAS}\tabAmax\tabAcw{IFS}\tabAmax\tabAcw{VRS}\tabAmax\tabAcw{VQR}\tabAmax\tabAcw{SEM}\tabAmax\tabAcw{00.000}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{w/o dependencies}\tabAmax\tabAmw{w/o inversion}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{Method}
\tabAtabular{l|ccc|c|c}{%
\toprule
\tabAname{{Method}} & \tabAcell{{UAS}} & \tabAcell{{IFS}} & \tabAcell{{VRS}} & \tabAcell{{VQR}} & \tabAcell{{SEM}} \\
\midrule
\tabAname{{w/o dependencies}} & \tabAcell{{68.9}} & \tabAcell{{87.6}} & \tabAcell{{81.8}} & \tabAcell{{4.24}} & \tabAcell{{93.6}} \\
\tabAname{{w/o inversion}} & \tabAcell{{73.2}} & \tabAcell{{90.1}} & \tabAcell{{85.9}} & \tabAcell{{4.35}} & \tabAcell{{88.9}} \\
\tabAtileF{tabAours}{\tabAmw}{l}{{\textbf{Ours}}} & \tabAtile{tabAours}{\tabAcw}{c}{{79.8}} & \tabAtile{tabAours}{\tabAcw}{c}{{91.7}} & \tabAtile{tabAours}{\tabAcw}{c}{{90.1}} & \tabAtile{tabAours}{\tabAcw}{c}{{4.23}} & \tabAtile{tabAours}{\tabAcw}{c}{{93.5}} \\
\bottomrule}
\caption{Ablation of the causal components on CoVEBench editing. Without dependencies, the agent changes only the concept named in the instruction. Without inversion, the video is regenerated under newly sampled noise. Higher is better for all metrics.}
\label{tab:causal_ablation}
\end{table}


==> tables/category.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{Bg.}\tabAmax\tabAcw{Cam.}\tabAmax\tabAcw{Mot.}\tabAmax\tabAcw{Pos.}\tabAmax\tabAcw{Sty.}\tabAmax\tabAcw{Subj.}\tabAmax\tabAcw{VFX}\tabAmax\tabAcw{All}\tabAmax\tabAcw{\textbf{00.0}}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{w/o Causal Diorama}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{Method}
\tabAtabular{l|ccccccc|c}{%
\toprule
\tabAname{Method} & \tabAcell{Bg.} & \tabAcell{Cam.} & \tabAcell{Mot.} & \tabAcell{Pos.} & \tabAcell{Sty.} & \tabAcell{Subj.} & \tabAcell{VFX} & \tabAcell{All} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{UAS}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{w/o Causal Diorama} & \tabAcell{80.1} & \tabAcell{79.5} & \tabAcell{78.6} & \tabAcell{77.4} & \tabAcell{79.5} & \tabAcell{77.5} & \tabAcell{77.5} & \tabAcell{78.0} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{84.2}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{80.4}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{79.7}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{78.6}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{81.1}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{80.4}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{77.8}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{79.8}} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{SEM}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{w/o Causal Diorama} & \tabAcell{61.8} & \tabAcell{54.8} & \tabAcell{52.2} & \tabAcell{53.4} & \tabAcell{61.9} & \tabAcell{55.0} & \tabAcell{53.9} & \tabAcell{55.5} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{92.5}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{92.2}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{93.2}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{90.1}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{88.5}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{94.6}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{90.0}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{93.5}} \\
\bottomrule}
\caption{Per-category results of editing real videos on CoVEBench. The variant without the Causal Diorama replaces it with text and keeps the rest of the procedure, as in \Cref{tab:ablation}. The columns are the official categories, background (Bg.), camera (Cam.), motion (Mot.), position (Pos.), style (Sty.), subject (Subj.)\ and visual effects (VFX), plus all instructions (All). An instruction counts in every category it involves. Higher is better.}
\label{tab:category}
\end{table}


==> tables/compbench.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.4pt}\renewcommand{\arraystretch}{1.12}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{Cons.}\tabAmax\tabAcw{Dyn.}\tabAmax\tabAcw{Spat.}\tabAmax\tabAcw{Mot.}\tabAmax\tabAcw{Act.}\tabAmax\tabAcw{Inter.}\tabAmax\tabAcw{Num.}\tabAmax\tabAcw{Avg.}\tabAmax\tabAcw{\textbf{.000}}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{Dreamina 1.2~\cite{capcut2024dreamina}}\tabAmax\tabAmw{Kling 1.0~\cite{kuaishou2024kling}}\tabAmax\tabAmw{Veo 3.1~\cite{google2025veo}}\tabAmax\tabAmw{PixVerse V3~\cite{pixverse2024}}\tabAmax\tabAmw{LTX 2.3~\cite{hacohen2026ltx2}}\tabAmax\tabAmw{MiniMax H3~\cite{minimax2026h3}}\tabAmax\tabAmw{Wan2.2 A14B~\cite{wan2025wan}}\tabAmax\tabAmw{Comp-Attn~\cite{zhang2026compattn}}\tabAmax\tabAmw{AVG~\cite{hassan2025avg}}\tabAmax\tabAmw{CAPE-T2V~\cite{jia2026cape}}\tabAmax\tabAmw{AVG~\cite{hassan2025avg}}\tabAmax\tabAmw{CWM~\cite{chen2026cwm}}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{\textit{Commercial}}\tabAmax\tabAmw{\textit{Open-source}}\tabAmax\tabAmw{\textit{On Wan2.2 A14B}}\tabAmax\tabAmw{\textit{On MiniMax H3}}\tabAmax\tabAmw{Method}
\tabAtabular{l|ccccccc|c}{%
\toprule
\tabAname{Method} & \tabAcell{Cons.} & \tabAcell{Dyn.} & \tabAcell{Spat.} & \tabAcell{Mot.} & \tabAcell{Act.} & \tabAcell{Inter.} & \tabAcell{Num.} & \tabAcell{Avg.} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Commercial}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{Dreamina 1.2~\cite{capcut2024dreamina}} & \tabAcell{.691} & \tabAcell{.005} & \tabAcell{.577} & \tabAcell{.236} & \tabAcell{.592} & \tabAcell{.682} & \tabAcell{.438} & \tabAcell{.460} \\
\tabAname{Kling 1.0~\cite{kuaishou2024kling}} & \tabAcell{.693} & \tabAcell{.010} & \tabAcell{.569} & \tabAcell{.256} & \tabAcell{.579} & \tabAcell{.713} & \tabAcell{.441} & \tabAcell{.466} \\
\tabAname{Veo 3.1~\cite{google2025veo}} & \tabAcell{.765} & \tabAcell{.257} & \tabAcell{.598} & \tabAcell{.512} & \tabAcell{.718} & \tabAcell{.629} & \tabAcell{.438} & \tabAcell{.559} \\
\tabAname{PixVerse V3~\cite{pixverse2024}} & \tabAcell{.706} & \tabAcell{.062} & \tabAcell{.598} & \tabAcell{.287} & \tabAcell{\textbf{.872}} & \tabAcell{.831} & \tabAcell{.607} & \tabAcell{.566} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Open-source}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{LTX 2.3~\cite{hacohen2026ltx2}} & \tabAcell{.791} & \tabAcell{.109} & \tabAcell{.530} & \tabAcell{.270} & \tabAcell{.520} & \tabAcell{.469} & \tabAcell{.281} & \tabAcell{.424} \\
\tabAname{MiniMax H3~\cite{minimax2026h3}} & \tabAcell{.786} & \tabAcell{.228} & \tabAcell{.641} & \tabAcell{.279} & \tabAcell{.681} & \tabAcell{.565} & \tabAcell{.320} & \tabAcell{.500} \\
\tabAname{Wan2.2 A14B~\cite{wan2025wan}} & \tabAcell{.839} & \tabAcell{.126} & \tabAcell{.662} & \tabAcell{.365} & \tabAcell{.753} & \tabAcell{.790} & \tabAcell{.484} & \tabAcell{.574} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{On Wan2.2 A14B}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{Comp-Attn~\cite{zhang2026compattn}} & \tabAcell{.873} & \tabAcell{.132} & \tabAcell{.724} & \tabAcell{.471} & \tabAcell{.854} & \tabAcell{.860} & \tabAcell{.577} & \tabAcell{.641} \\
\tabAname{AVG~\cite{hassan2025avg}} & \tabAcell{.927} & \tabAcell{.217} & \tabAcell{.680} & \tabAcell{.320} & \tabAcell{.850} & \tabAcell{\textbf{.886}} & \tabAcell{.781} & \tabAcell{.666} \\
\tabAname{CAPE-T2V~\cite{jia2026cape}} & \tabAcell{.910} & \tabAcell{.306} & \tabAcell{.704} & \tabAcell{.488} & \tabAcell{.810} & \tabAcell{.819} & \tabAcell{.628} & \tabAcell{.667} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{On MiniMax H3}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{AVG~\cite{hassan2025avg}} & \tabAcell{\textbf{.939}} & \tabAcell{.257} & \tabAcell{.750} & \tabAcell{.367} & \tabAcell{.804} & \tabAcell{.704} & \tabAcell{.684} & \tabAcell{.644} \\
\tabAname{CWM~\cite{chen2026cwm}} & \tabAcell{.840} & \tabAcell{.321} & \tabAcell{\textbf{.783}} & \tabAcell{.515} & \tabAcell{.683} & \tabAcell{.711} & \tabAcell{.778} & \tabAcell{.662} \\
\midrule
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{.936} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{.330}} & \tabAtile{tabAours}{\tabAcw}{c}{.777} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{.599}} & \tabAtile{tabAours}{\tabAcw}{c}{.793} & \tabAtile{tabAours}{\tabAcw}{c}{.737} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{.912}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{.726}} \\
\bottomrule}
\caption{Generation from text on T2V-CompBench. Each column is a category of tasks, scored from 0 to 1 with the leading zero omitted. Higher is better, and bold numbers mark the best result.}
\label{tab:compbench}
\end{table}


==> tables/covebench_common.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{UAS}\tabAmax\tabAcw{IFS}\tabAmax\tabAcw{VRS}\tabAmax\tabAcw{VQR}\tabAmax\tabAcw{SEM}\tabAmax\tabAcw{\textbf{0.000}}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{Kling 3.0 Omni~\cite{kuaishou2026kling3omni}}\tabAmax\tabAmw{Seedance 2.0~\cite{seedance2026v2}}\tabAmax\tabAmw{\textit{Shared with Kling 3.0 Omni}}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{Method}
\tabAtabular{l|ccc|c|c}{%
\toprule
\tabAname{Method} & \tabAcell{UAS} & \tabAcell{IFS} & \tabAcell{VRS} & \tabAcell{VQR} & \tabAcell{SEM} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Shared with Kling 3.0 Omni}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{Kling 3.0 Omni~\cite{kuaishou2026kling3omni}} & \tabAcell{53.30} & \tabAcell{74.97} & \tabAcell{73.70} & \tabAcell{4.217} & \tabAcell{\textbf{95.72}} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{80.06}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{91.69}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{89.65}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{4.301}} & \tabAtile{tabAours}{\tabAcw}{c}{93.18} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Shared with Seedance 2.0}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{Seedance 2.0~\cite{seedance2026v2}} & \tabAcell{59.62} & \tabAcell{77.94} & \tabAcell{78.51} & \tabAcell{4.208} & \tabAcell{\textbf{95.14}} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{79.17}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{91.72}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{89.50}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{4.216}} & \tabAtile{tabAours}{\tabAcw}{c}{92.46} \\
\bottomrule}
\caption{Editing of real videos on the CoVEBench videos that our method shares with Kling 3.0 Omni and with Seedance 2.0. Bold numbers mark the better result in each block, and higher is better for all metrics.}
\label{tab:common}
\end{table}


==> tables/covebench_edit.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\definecolor{tabArk}{RGB}{105,105,105}%
\makeatletter
\@ifundefined{tabArw}{\newlength\tabArw\newlength\tabAaw\newlength\tabAtmp}{}
\@ifundefined{tabAgw}{\newlength\tabAgw}{}%
\@ifundefined{tabAyw}{\newlength\tabAyw}{}%
\makeatother
\def\tabAcellW#1#2{\makebox[#1]{\tabAtext{#2}}}
\def\tabArkc#1{\textcolor{tabArk}{#1}}
\def\tabAgwfit#1{\settowidth\tabAtmp{#1}\addtolength\tabAtmp{-\tabArw}\addtolength\tabAtmp{-2\tabcolsep}%
  \ifdim\tabAtmp>\tabAgw\setlength\tabAgw{\tabAtmp}\fi}
\begin{table*}[t]
\centering
\normalsize
\setlength{\tabcolsep}{5.5pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{\textbf{UAS}$\uparrow$}\tabAmax\tabAcw{\textbf{IFS}$\uparrow$}\tabAmax\tabAcw{\textbf{VRS}$\uparrow$}\tabAmax\tabAcw{\textbf{VQR}$\uparrow$}\tabAmax\tabAcw{\textbf{SEM}$\uparrow$}\tabAmax\tabAcw{\textbf{00.000}}
\setlength\tabAyw{0pt}\tabAmax\tabAyw{Year}\tabAmax\tabAyw{2024}\tabAmax\tabAyw{2025}\tabAmax\tabAyw{2026}
\setlength\tabArw{0pt}\tabAmax\tabArw{Rank$\downarrow$}\tabAmax\tabArw{1}\tabAmax\tabArw{2}\tabAmax\tabArw{3}\tabAmax\tabArw{4}\tabAmax\tabArw{5}\tabAmax\tabArw{6}\tabAmax\tabArw{7}\tabAmax\tabArw{8}\tabAmax\tabArw{9}\tabAmax\tabArw{10}\tabAmax\tabArw{11}\tabAmax\tabArw{12}\tabAmax\tabArw{13}\tabAmax\tabArw{14}
\setlength\tabAgw{\tabAcw}\tabAgwfit{Video quality}\tabAgwfit{Video fidelity}
\setlength\tabAaw{0pt}\tabAmax\tabAaw{Avg.\ Rank$\downarrow$}\tabAmax\tabAaw{\textbf{00.00}}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{Kling 3.0 Omni$^\dagger$~\cite{kuaishou2026kling3omni}}\tabAmax\tabAmw{HappyHorse 1.0~\cite{happyhorse2026}}\tabAmax\tabAmw{Wan2.7~\cite{alibaba2026wan27}}\tabAmax\tabAmw{Seedance 2.0$^\dagger$~\cite{seedance2026v2}}\tabAmax\tabAmw{VACE~\cite{jiang2025vace}}\tabAmax\tabAmw{InsV2V~\cite{cheng2024insv2v}}\tabAmax\tabAmw{ReCo~\cite{zhang2025reco}}\tabAmax\tabAmw{ICVE~\cite{liao2025icve}}\tabAmax\tabAmw{Lucy-Edit~\cite{decart2025lucyedit}}\tabAmax\tabAmw{Ditto~\cite{bai2025ditto}}\tabAmax\tabAmw{Kiwi~\cite{lin2026kiwiedit}}\tabAmax\tabAmw{OmniWeaving~\cite{pan2026omniweaving}}\tabAmax\tabAmw{Bernini~\cite{bernini2026}}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{\textit{Commercial}}\tabAmax\tabAmw{\textit{Open-source}}\tabAmax\tabAmw{Method}
\tabAtabular{lc|cccc|cc|cc|c}{%
\toprule
\tabAname{} & \tabAcellW{\tabAyw}{} & \multicolumn{4}{c|}{\tabAtext{Instruction compliance}} & \multicolumn{2}{c|}{\tabAtext{Video quality}} & \multicolumn{2}{c|}{\tabAtext{Video fidelity}} & \\
\cline{3-6}\cline{7-8}\cline{9-10}
\tabAname{\raisebox{7pt}[0pt][0pt]{Method}} & \tabAcellW{\tabAyw}{\raisebox{7pt}[0pt][0pt]{Year}} & \tabAcellW{\tabArw}{Rank$\downarrow$} & \tabAcell{UAS$\uparrow$} & \tabAcell{IFS$\uparrow$} & \tabAcell{VRS$\uparrow$} & \tabAcellW{\tabArw}{Rank$\downarrow$} & \tabAcellW{\tabAgw}{VQR$\uparrow$} & \tabAcellW{\tabArw}{Rank$\downarrow$} & \tabAcellW{\tabAgw}{SEM$\uparrow$} & \tabAcellW{\tabAaw}{\raisebox{7pt}[0pt][0pt]{Avg.\ Rank$\downarrow$}} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Commercial}} & \tabAtile{tabAband}{\tabAyw}{c}{} & \tabAtile{tabAband}{\tabArw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabArw}{c}{} & \tabAtile{tabAband}{\tabAgw}{c}{} & \tabAtile{tabAband}{\tabArw}{c}{} & \tabAtile{tabAband}{\tabAgw}{c}{} & \tabAtile{tabAband}{\tabAaw}{c}{} \\
\tabAname{Kling 3.0 Omni$^\dagger$~\cite{kuaishou2026kling3omni}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{6}} & \tabAcell{53.30} & \tabAcell{74.97} & \tabAcell{73.70} & \tabAcellW{\tabArw}{\tabArkc{4}} & \tabAcellW{\tabAgw}{4.217} & \tabAcellW{\tabArw}{\tabArkc{1}} & \tabAcellW{\tabAgw}{\textbf{95.72}} & \tabAcellW{\tabAaw}{3.67} \\
\tabAname{HappyHorse 1.0~\cite{happyhorse2026}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{5}} & \tabAcell{55.18} & \tabAcell{76.54} & \tabAcell{84.52} & \tabAcellW{\tabArw}{\tabArkc{2}} & \tabAcellW{\tabAgw}{4.388} & \tabAcellW{\tabArw}{\tabArkc{4}} & \tabAcellW{\tabAgw}{92.73} & \tabAcellW{\tabAaw}{3.67} \\
\tabAname{Wan2.7~\cite{alibaba2026wan27}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{4}} & \tabAcell{56.89} & \tabAcell{82.02} & \tabAcell{79.97} & \tabAcellW{\tabArw}{\tabArkc{1}} & \tabAcellW{\tabAgw}{\textbf{4.407}} & \tabAcellW{\tabArw}{\tabArkc{6}} & \tabAcellW{\tabAgw}{87.90} & \tabAcellW{\tabAaw}{3.67} \\
\tabAname{Seedance 2.0$^\dagger$~\cite{seedance2026v2}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{3}} & \tabAcell{59.62} & \tabAcell{77.94} & \tabAcell{78.51} & \tabAcellW{\tabArw}{\tabArkc{5}} & \tabAcellW{\tabAgw}{4.208} & \tabAcellW{\tabArw}{\tabArkc{2}} & \tabAcellW{\tabAgw}{95.14} & \tabAcellW{\tabAaw}{3.33} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Open-source}} & \tabAtile{tabAband}{\tabAyw}{c}{} & \tabAtile{tabAband}{\tabArw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabArw}{c}{} & \tabAtile{tabAband}{\tabAgw}{c}{} & \tabAtile{tabAband}{\tabArw}{c}{} & \tabAtile{tabAband}{\tabAgw}{c}{} & \tabAtile{tabAband}{\tabAaw}{c}{} \\
\tabAname{VACE~\cite{jiang2025vace}} & \tabAcellW{\tabAyw}{2025} & \tabAcellW{\tabArw}{\tabArkc{14}} & \tabAcell{9.69} & \tabAcell{22.92} & \tabAcell{41.35} & \tabAcellW{\tabArw}{\tabArkc{8}} & \tabAcellW{\tabAgw}{3.718} & \tabAcellW{\tabArw}{\tabArkc{9}} & \tabAcellW{\tabAgw}{81.73} & \tabAcellW{\tabAaw}{10.33} \\
\tabAname{InsV2V~\cite{cheng2024insv2v}} & \tabAcellW{\tabAyw}{2024} & \tabAcellW{\tabArw}{\tabArkc{13}} & \tabAcell{14.61} & \tabAcell{37.18} & \tabAcell{47.36} & \tabAcellW{\tabArw}{\tabArkc{12}} & \tabAcellW{\tabAgw}{3.307} & \tabAcellW{\tabArw}{\tabArkc{11}} & \tabAcellW{\tabAgw}{77.85} & \tabAcellW{\tabAaw}{12.00} \\
\tabAname{ReCo~\cite{zhang2025reco}} & \tabAcellW{\tabAyw}{2025} & \tabAcellW{\tabArw}{\tabArkc{12}} & \tabAcell{24.35} & \tabAcell{54.16} & \tabAcell{47.42} & \tabAcellW{\tabArw}{\tabArkc{14}} & \tabAcellW{\tabAgw}{3.146} & \tabAcellW{\tabArw}{\tabArkc{13}} & \tabAcellW{\tabAgw}{70.03} & \tabAcellW{\tabAaw}{13.00} \\
\tabAname{ICVE~\cite{liao2025icve}} & \tabAcellW{\tabAyw}{2025} & \tabAcellW{\tabArw}{\tabArkc{11}} & \tabAcell{25.83} & \tabAcell{53.14} & \tabAcell{54.00} & \tabAcellW{\tabArw}{\tabArkc{13}} & \tabAcellW{\tabAgw}{3.277} & \tabAcellW{\tabArw}{\tabArkc{12}} & \tabAcellW{\tabAgw}{71.02} & \tabAcellW{\tabAaw}{12.00} \\
\tabAname{Lucy-Edit~\cite{decart2025lucyedit}} & \tabAcellW{\tabAyw}{2025} & \tabAcellW{\tabArw}{\tabArkc{10}} & \tabAcell{26.01} & \tabAcell{50.85} & \tabAcell{58.68} & \tabAcellW{\tabArw}{\tabArkc{9}} & \tabAcellW{\tabAgw}{3.688} & \tabAcellW{\tabArw}{\tabArkc{7}} & \tabAcellW{\tabAgw}{86.13} & \tabAcellW{\tabAaw}{8.67} \\
\tabAname{Ditto~\cite{bai2025ditto}} & \tabAcellW{\tabAyw}{2025} & \tabAcellW{\tabArw}{\tabArkc{9}} & \tabAcell{26.50} & \tabAcell{49.45} & \tabAcell{60.69} & \tabAcellW{\tabArw}{\tabArkc{7}} & \tabAcellW{\tabAgw}{3.921} & \tabAcellW{\tabArw}{\tabArkc{14}} & \tabAcellW{\tabAgw}{58.02} & \tabAcellW{\tabAaw}{10.00} \\
\tabAname{Kiwi~\cite{lin2026kiwiedit}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{8}} & \tabAcell{29.03} & \tabAcell{53.90} & \tabAcell{56.13} & \tabAcellW{\tabArw}{\tabArkc{10}} & \tabAcellW{\tabAgw}{3.670} & \tabAcellW{\tabArw}{\tabArkc{10}} & \tabAcellW{\tabAgw}{79.51} & \tabAcellW{\tabAaw}{9.33} \\
\tabAname{OmniWeaving~\cite{pan2026omniweaving}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{7}} & \tabAcell{30.14} & \tabAcell{57.18} & \tabAcell{61.75} & \tabAcellW{\tabArw}{\tabArkc{11}} & \tabAcellW{\tabAgw}{3.660} & \tabAcellW{\tabArw}{\tabArkc{8}} & \tabAcellW{\tabAgw}{85.05} & \tabAcellW{\tabAaw}{8.67} \\
\tabAname{Bernini~\cite{bernini2026}} & \tabAcellW{\tabAyw}{2026} & \tabAcellW{\tabArw}{\tabArkc{2}} & \tabAcell{65.34} & \tabAcell{82.78} & \tabAcell{80.63} & \tabAcellW{\tabArw}{\tabArkc{6}} & \tabAcellW{\tabAgw}{4.049} & \tabAcellW{\tabArw}{\tabArkc{5}} & \tabAcellW{\tabAgw}{89.34} & \tabAcellW{\tabAaw}{4.33} \\
\midrule
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAyw}{c}{\textcolor{black!45}{--}} & \tabAtile{tabAours}{\tabArw}{c}{\tabArkc{1}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{79.78}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{91.73}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{90.11}} & \tabAtile{tabAours}{\tabArw}{c}{\tabArkc{3}} & \tabAtile{tabAours}{\tabAgw}{c}{4.227} & \tabAtile{tabAours}{\tabArw}{c}{\tabArkc{3}} & \tabAtile{tabAours}{\tabAgw}{c}{93.46} & \tabAtile{tabAours}{\tabAaw}{c}{\textbf{2.33}} \\
\bottomrule}
\caption{Editing of real videos on CoVEBench. Rank gives the rank of each method on the primary metric of each dimension, and Avg.\ Rank is their mean. Bold numbers mark the best result in each column. $^\dagger$Kling 3.0 Omni and Seedance 2.0 are evaluated on 334 and 410 videos, respectively, as the remaining videos cannot be processed due to the length, format and content restrictions of their APIs.}
\label{tab:covebench_edit}
\vspace{-10pt}
\end{table*}


==> tables/covebench_rev.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{\textbf{UAS}}\tabAmax\tabAcw{\textbf{IFS}}\tabAmax\tabAcw{\textbf{VRS}}\tabAmax\tabAcw{\textbf{VQR}}\tabAmax\tabAcw{\textbf{SEM}}\tabAmax\tabAcw{\textbf{00.000}}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{Lucy-Edit~\cite{decart2025lucyedit}}\tabAmax\tabAmw{Kiwi~\cite{lin2026kiwiedit}}\tabAmax\tabAmw{Ditto~\cite{bai2025ditto}}\tabAmax\tabAmw{OmniWeaving~\cite{pan2026omniweaving}}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{\textit{Open-source}}\tabAmax\tabAmw{Method}
\tabAtabular{l|ccc|c|c}{%
\toprule
\tabAname{Method} & \tabAcell{UAS} & \tabAcell{IFS} & \tabAcell{VRS} & \tabAcell{VQR} & \tabAcell{SEM} \\
\midrule
\tabAname{Lucy-Edit~\cite{decart2025lucyedit}} & \tabAcell{26.4} & \tabAcell{49.1} & \tabAcell{52.6} & \tabAcell{3.63} & \tabAcell{84.8} \\
\tabAname{Kiwi~\cite{lin2026kiwiedit}} & \tabAcell{29.0} & \tabAcell{50.1} & \tabAcell{51.1} & \tabAcell{4.06} & \tabAcell{95.1} \\
\tabAname{Ditto~\cite{bai2025ditto}} & \tabAcell{29.6} & \tabAcell{50.9} & \tabAcell{53.3} & \tabAcell{4.16} & \tabAcell{70.1} \\
\tabAname{OmniWeaving~\cite{pan2026omniweaving}} & \tabAcell{32.3} & \tabAcell{55.9} & \tabAcell{56.2} & \tabAcell{3.87} & \tabAcell{84.4} \\
\midrule
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{79.5}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{92.7}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{89.7}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{4.30}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{95.3}} \\
\bottomrule}
\caption{Revision of generated videos on CoVEBench. Higher is better, and bold numbers mark the best result in each column.}
\label{tab:covebench_rev}
\vspace{-12pt}
\end{table}


==> tables/openve.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\makeatletter\@ifundefined{tabAow}{\newlength\tabAow}{}\makeatother%
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1.8pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}%
\let\rk\tabArk\let\rkO\tabArkO
\setlength\tabAcw{0pt}\tabAmax\tabAcw{Style}\tabAmax\tabAcw{Bkg.}\tabAmax\tabAcw{Chg.}\tabAmax\tabAcw{Rem.}\tabAmax\tabAcw{Add}\tabAmax\tabAcw{Sub.}\tabAmax\tabAcw{Cam.}\tabAmax\tabAcw{Cre.}\tabAmax\tabAcw{\textbf{0.00}}
\setlength\tabAow{\tabAcw}\tabAmax\tabAow{Overall}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{Runway Aleph~\cite{runway2025aleph}}\tabAmax\tabAmw{Kling O1~\cite{kling2025omni}}\tabAmax\tabAmw{PixVerse R1~\cite{pixverse2026r1}}\tabAmax\tabAmw{Ditto~\cite{bai2025ditto}}\tabAmax\tabAmw{Lucy-Edit~\cite{decart2025lucyedit}}\tabAmax\tabAmw{OpenVE-Edit~\cite{he2026openve}}\tabAmax\tabAmw{Kiwi~\cite{lin2026kiwiedit}}\tabAmax\tabAmw{OmniWeaving~\cite{pan2026omniweaving}}\tabAmax\tabAmw{Aurora~\cite{yu2026aurora}}\tabAmax\tabAmw{VINO~\cite{chen2026vino}}\tabAmax\tabAmw{Bernini~\cite{bernini2026}}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{\textit{Commercial}}\tabAmax\tabAmw{\textit{Open-source}}\tabAmax\tabAmw{Method}
\tabAtabular{l|cccccccc|c}{%
\toprule
\tabAname{Method} & \tabAcell{Style} & \tabAcell{Bkg.} & \tabAcell{Chg.} & \tabAcell{Rem.} & \tabAcell{Add} & \tabAcell{Sub.} & \tabAcell{Cam.} & \tabAcell{Cre.} & {\setlength\tabAcw{\tabAow}\tabAcell{Overall}} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Commercial}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAow}{c}{} \\
\tabAname{Runway Aleph~\cite{runway2025aleph}} & \rk{0}{3.72} & \rk{0}{2.62} & \rk{0}{4.18} & \rk{1}{4.16} & \rk{0}{2.78} & \rk{0}{3.62} & \rk{1}{4.53} & \rk{0}{3.64} & {\setlength\tabAcw{\tabAow}\rk{0}{3.62}} \\
\tabAname{Kling O1~\cite{kling2025omni}} & \rk{0}{4.34} & \rk{0}{3.38} & \rk{0}{4.44} & \rk{0}{3.23} & \rk{0}{3.32} & \rk{0}{3.62} & \tabAna & \rk{0}{3.49} & {\setlength\tabAcw{\tabAow}\rk{0}{3.71}} \\
\tabAname{PixVerse R1~\cite{pixverse2026r1}} & \rk{0}{3.29} & \rk{0}{3.02} & \rk{0}{4.10} & \rk{0}{2.33} & \rk{0}{2.82} & \rk{0}{2.69} & \tabAna & \rk{0}{3.09} & {\setlength\tabAcw{\tabAow}\rk{0}{3.06}} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{Open-source}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAow}{c}{} \\
\tabAname{Ditto~\cite{bai2025ditto}} & \rk{0}{4.01} & \rk{0}{1.68} & \rk{0}{2.03} & \rk{0}{1.53} & \rk{0}{1.41} & \rk{0}{2.81} & \rk{0}{1.32} & \rk{0}{1.23} & {\setlength\tabAcw{\tabAow}\rk{0}{2.05}} \\
\tabAname{Lucy-Edit~\cite{decart2025lucyedit}} & \rk{0}{2.27} & \rk{0}{1.57} & \rk{0}{3.20} & \rk{0}{1.75} & \rk{0}{2.30} & \rk{0}{1.61} & \rk{0}{1.61} & \rk{0}{2.86} & {\setlength\tabAcw{\tabAow}\rk{0}{2.15}} \\
\tabAname{OpenVE-Edit~\cite{he2026openve}} & \rk{0}{3.16} & \rk{0}{2.36} & \rk{0}{2.98} & \rk{0}{1.85} & \rk{0}{2.15} & \rk{0}{2.91} & \rk{0}{2.02} & \rk{0}{2.31} & {\setlength\tabAcw{\tabAow}\rk{0}{2.49}} \\
\tabAname{Kiwi~\cite{lin2026kiwiedit}} & \rk{0}{3.72} & \rk{0}{2.67} & \rk{0}{3.91} & \rk{0}{2.69} & \rk{0}{2.55} & \tabAna & \tabAna & \tabAna & {\setlength\tabAcw{\tabAow}\rk{0}{3.11}} \\
\tabAname{OmniWeaving~\cite{pan2026omniweaving}} & \rk{0}{3.91} & \rk{0}{2.30} & \rk{0}{3.65} & \rk{0}{3.22} & \rk{0}{2.30} & \rk{0}{3.53} & \tabAna & \tabAna & {\setlength\tabAcw{\tabAow}\rk{0}{3.13}} \\
\tabAname{Aurora~\cite{yu2026aurora}} & \rk{0}{4.07} & \rk{0}{2.67} & \rk{0}{4.03} & \rk{0}{3.73} & \rk{0}{2.78} & \rk{0}{2.97} & \tabAna & \tabAna & {\setlength\tabAcw{\tabAow}\rk{0}{3.38}} \\
\tabAname{VINO~\cite{chen2026vino}} & \rk{0}{4.34} & \rk{0}{2.54} & \rk{0}{3.73} & \rk{0}{3.22} & \rk{0}{2.77} & \rk{0}{2.61} & \rk{0}{2.81} & \rk{0}{3.29} & {\setlength\tabAcw{\tabAow}\rk{0}{3.18}} \\
\tabAname{Bernini~\cite{bernini2026}} & \rk{0}{4.29} & \rk{1}{3.58} & \rk{1}{4.72} & \rk{0}{4.10} & \rk{1}{3.35} & \rk{0}{3.55} & \rk{0}{4.18} & \rk{0}{3.84} & {\setlength\tabAcw{\tabAow}\rk{0}{3.96}} \\
\midrule
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \rkO{1}{4.66} & \rkO{0}{3.39} & \rkO{0}{4.32} & \rkO{0}{3.77} & \rkO{0}{3.32} & \rkO{1}{4.27} & \rkO{0}{4.47} & \rkO{1}{4.07} & {\setlength\tabAcw{\tabAow}\rkO{1}{4.00}} \\
\bottomrule}
\caption{Editing of real videos on OpenVE-Bench. Each column is a category of tasks, and Overall averages them weighted by their numbers of pairs. -- marks categories not evaluated by the source, and bold numbers mark the best result in each column.}
\label{tab:openve}
\vspace{-18pt}
\end{table}


==> tables/threshold.tex <==
\definecolor{tabAband}{RGB}{238,243,248}%
\definecolor{tabAours}{RGB}{236,236,236}%
\makeatletter
\@ifundefined{tabAcw}{\newlength\tabAcw\newlength\tabAmw}{}
\def\tabAmax#1#2{\settowidth\@tempdima{#2}\ifdim\@tempdima>#1\setlength#1{\@tempdima}\fi}
\long\def\tabAtabular#1#2{\leavevmode
  \rlap{\def\tabA@pass{1}\tabA@inkless\begin{tabular}{#1}#2\end{tabular}}%
  {\def\tabA@pass{2}\begin{tabular}{#1}#2\end{tabular}}}
\def\tabA@pass{0}
\def\tabA@inkless{\@ifundefined{ver@array.sty}{}{\edef\vline{\hskip\the\arrayrulewidth}}%
  \arrayrulewidth\z@ \advance\abovetopsep\heavyrulewidth \advance\aboverulesep\lightrulewidth
  \advance\belowbottomsep\heavyrulewidth \advance\belowbottomsep-\lightrulewidth
  \heavyrulewidth\z@ \lightrulewidth\z@}
\def\tabAeps{.15pt}
\def\tabA@tile#1#2#3#4#5#6{\ifnum\tabA@pass=\tw@\makebox[#4][#5]{#6}\else
  \hspace*{\dimexpr-\tabcolsep-#1\relax}%
  \rlap{\smash{\color{#3}\vrule width\dimexpr#4+2\tabcolsep+#1\relax
    height\dimexpr\ht\@arstrutbox+#2\relax depth\dp\@arstrutbox}}%
  \hspace*{\dimexpr\tabcolsep+#1\relax}\makebox[#4][#5]{\tabAtext{#6}}\fi}
\def\tabAtile{\tabA@tile\tabAeps\z@}
\def\tabAtileU{\tabA@tile\tabAeps\tabAeps}
\def\tabAtileF{\tabA@tile\z@\z@}
\def\tabAtext#1{\ifnum\tabA@pass=\@ne\phantom{#1}\else#1\fi}
\def\tabAcell#1{\makebox[\tabAcw]{\tabAtext{#1}}}
\def\tabAname#1{\makebox[\tabAmw][l]{\tabAtext{#1}}}
\def\tabAna{\tabAcell{\textcolor{black!45}{--}}}
\def\tabAmark#1#2{\ifcase#1\relax#2\or\textbf{#2}\or\textit{#2}\or\underline{#2}\fi}
\def\tabArk#1#2{\tabAcell{\tabAmark{#1}{#2}}}
\def\tabArkO#1#2{\tabAtile{tabAours}{\tabAcw}{c}{\tabAmark{#1}{#2}}}
\makeatother
\definecolor{tabAprim}{RGB}{252,244,222}%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.16}
\setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}
\setlength\tabAcw{0pt}\tabAmax\tabAcw{50}\tabAmax\tabAcw{60}\tabAmax\tabAcw{70}\tabAmax\tabAcw{80}\tabAmax\tabAcw{90}\tabAmax\tabAcw{\textbf{00.0}}
\setlength\tabAmw{0pt}\tabAmax\tabAmw{MiniMax H3~\cite{minimax2026h3}}\tabAmax\tabAmw{w/o Causal Diorama}\tabAmax\tabAmw{\textbf{Ours}}\tabAmax\tabAmw{Method}\tabAmax\tabAmw{\textit{UAS $\geq$ 50}}\tabAmax\tabAmw{\textit{UAS $=$ 100}}
\tabAtabular{l|ccccc}{%
\toprule
\tabAname{} & \multicolumn{5}{c}{\tabAtext{SEM $\geq$}} \\
\cline{2-6}
\tabAname{Method} & \tabAcell{50} & \tabAcell{60} & \tabAcell{70} & \tabAcell{80} & \tabAcell{90} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{UAS $\geq$ 50}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{MiniMax H3~\cite{minimax2026h3}} & \tabAcell{65.4} & \tabAcell{63.4} & \tabAcell{60.4} & \tabAcell{56.6} & \tabAcell{48.1} \\
\tabAname{w/o Causal Diorama} & \tabAcell{50.2} & \tabAcell{39.3} & \tabAcell{28.0} & \tabAcell{16.5} & \tabAcell{10.3} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{86.7}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{85.9}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{83.5}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{78.9}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{69.7}} \\
\midrule
\tabAtileF{tabAband}{\tabAmw}{l}{\textit{UAS $=$ 100}} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} & \tabAtile{tabAband}{\tabAcw}{c}{} \\
\tabAname{MiniMax H3~\cite{minimax2026h3}} & \tabAcell{38.6} & \tabAcell{37.6} & \tabAcell{36.4} & \tabAcell{34.6} & \tabAcell{29.1} \\
\tabAname{w/o Causal Diorama} & \tabAcell{33.4} & \tabAcell{26.6} & \tabAcell{19.3} & \tabAcell{12.6} & \tabAcell{8.5} \\
\tabAtileF{tabAours}{\tabAmw}{l}{\textbf{Ours}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{57.6}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{57.1}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{55.4}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{52.9}} & \tabAtile{tabAours}{\tabAcw}{c}{\textbf{47.6}} \\
\bottomrule}
\caption{Success rate (\%) of editing real videos on CoVEBench under different thresholds. A result counts as a success when its UAS and SEM both reach the given thresholds. All variants use MiniMax H3 as the generator, as in \Cref{tab:ablation}. Bold numbers mark the best result in each column.}
\label{tab:threshold}
\end{table}

